Muon identification in a compact single-layered water Cherenkov detector and gamma/hadron discrimination using Machine Learning techniques

The muon tagging is an essential tool to distinguish between gamma and hadron-induced showers in wide field-of-view gamma-ray observatories. In this work, it is shown that an efficient muon tagging (and counting) can be achieved using a water Cherenkov detector with a reduced water volume and 4 PMTs, provided that the PMT signal spatial and time patterns are interpreted by an analysis based on Machine Learning (ML). The developed analysis has been tested for different shower and array configurations. The output of the ML analysis, the probability of having a muon in the WCD station, has been used to notably discriminate between gamma and hadron induced showers with $S/ \sqrt{B} \sim 4$ for shower with energies $E_0 \sim1\,$TeV. Finally, for proton-induced showers, an estimator of the number of muons was built by means of the sum of the probabilities of having a muon in the stations. Resolutions about $20\%$ and a negligible bias are obtained for vertical showers with $N_{\mu} > 10$.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 1342 2019-01-29 17:20:57Z darko $

USEPDFLATEX := 1
USEBIBTEX := 1

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

